From loom spaces to veering triangulations

We introduce loom spaces, a generalisation of both the leaf spaces associated to pseudo-Anosov flows and the link spaces associated to veering triangulations. Following work of Gu\'eritaud, we prove that there is a locally veering triangulation canonically associated to every loom space, and that the realisation of this triangulation is homeomorphic to $\mathbb{R}^3$.

==> header_article.tex <==
%%% Environments %%%

% Numbering
% see http://tex.stackexchange.com/questions/41299/how-to-identify-the-counter-of-equation-theorem-and-section

\makeatletter
\let\c@equation\c@subsection
\makeatother
\numberwithin{equation}{section} 

\makeatletter
\let\c@figure\c@equation
\makeatother
\numberwithin{figure}{section} 

\makeatletter
\let\c@table\c@equation
\makeatother
\numberwithin{table}{section} 

%%% Turn off the above, and turn this on, for subsections to be numbered separately... 
%%% \numberwithin{equation}{section} 

% Formatting 
% see amsthdoc.pdf for general discussion. 

% \swapnumbers 

% It is Bourbaki style to put labels (numbering) before the <type>.
% This is used in various places - eg Dunfield recently, Bridson and
% Haefliger.  Suggested, but not used, by Bernstein
% (http://cr.yp.to/writing.html).  If you fix the non-bold/bold/italic
% problem (three typefaces in three words arrgh!) then it looks
% better.  But it doesn't match usage in the text, and I think that
% controls...  Perhaps if the numbers could be placed in the margin in
% a nice way?  But then there wuld be a ragged left.

\theoremstyle{plain}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{principle}[equation]{Principle}
\newtheorem{axiom}[equation]{Axiom}
\newtheorem{property}[equation]{Property}

\theoremstyle{definition}
\newtheorem{definition/}[equation]{Definition}
\newtheorem{problem}[equation]{Problem}
\newtheorem{solution}[equation]{Solution}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{example/}[equation]{Example}
\newtheorem{notation/}[equation]{Notation}
\newtheorem{fact}[equation]{Fact}
\newtheorem{question/}[equation]{Question}
\newtheorem*{question*}{Question}
\newtheorem*{answer*}{Answer}
\newtheorem*{application*}{Application}
\newtheorem{algorithm/}[equation]{Algorithm}
\newtheorem{objective}{Objective}[section]

%%% https://tex.stackexchange.com/questions/291346/marking-the-end-of-a-definition
%%% Using egreg's solution
\newenvironment{definition}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{definition/}}
  {\popQED\end{definition/}}

\newenvironment{example}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{example/}}
  {\popQED\end{example/}}

\newenvironment{notation}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{notation/}}
  {\popQED\end{notation/}}

\newenvironment{question}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{question/}}
  {\popQED\end{question/}}

\newenvironment{algorithm}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{algorithm/}}
  {\popQED\end{algorithm/}}

\theoremstyle{remark}
\newtheorem{remark/}[equation]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{case}{Case}
\newtheorem*{case*}{Case}
\renewcommand{\thecase}{\Roman{case}}
\newtheorem{claim}[equation]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem*{proofclaim}{Claim}
\newtheorem*{proofsubclaim}{Subclaim}

\newenvironment{remark}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{remark/}}
  {\popQED\end{remark/}}

%%% Refs
\newcommand{\refsec}[1]{Section~\ref{Sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{App:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{Thm:#1}}
\newcommand{\refcor}[1]{Corollary~\ref{Cor:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{Lem:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{Prop:#1}}
\newcommand{\refclm}[1]{Claim~\ref{Clm:#1}}
\newcommand{\refrem}[1]{Remark~\ref{Rem:#1}}
\newcommand{\refexa}[1]{Example~\ref{Exa:#1}}
\newcommand{\reffac}[1]{Fact~\ref{Fac:#1}}
\newcommand{\refexe}[1]{Exercise~\ref{Exe:#1}}
\newcommand{\refnot}[1]{Notation~\ref{Not:#1}}
\newcommand{\reffig}[1]{Figure~\ref{Fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{Tab:#1}}
\newcommand{\refdef}[1]{Definition~\ref{Def:#1}}
\newcommand{\refprob}[1]{Problem~\ref{Prob:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\refax}[1]{Axiom~\ref{Ax:#1}}
\newcommand{\refpro}[1]{Property~\ref{Pro:#1}}
\newcommand{\refrul}[1]{Rule~\ref{Rul:#1}}
\newcommand{\refque}[1]{Question~\ref{Que:#1}}
\newcommand{\refeqn}[1]{Equation~\ref{Eqn:#1}}
\newcommand{\refeqns}[1]{Equations~\ref{Eqns:#1}}
\newcommand{\refconj}[1]{Conjecture~\ref{Conj:#1}}
\newcommand{\refobj}[1]{Objective~\ref{Obj:#1}}
\newcommand{\refitm}[1]{(\ref{Itm:#1})}
\newcommand{\refcon}[1]{(\ref{Con:#1})} % conclusion

%%% Old

%% \newenvironment{solution}
%%   {\begin{proof}[Solution]}
%%   {\end{proof}}

%% \newenvironment{answer}
%%   {\begin{proof}[Answer]}
%%   {\end{proof}}


